Healing Products of Gaussian Processes

Gaussian processes (GPs) are nonparametric Bayesian models that have been applied to regression and classification problems. One of the approaches to alleviate their cubic training cost is the use of local GP experts trained on subsets of the data. In particular, product-of-expert models combine the predictive distributions of local experts through a tractable product operation. While these expert models allow for massively distributed computation, their predictions typically suffer from erratic behaviour of the mean or uncalibrated uncertainty quantification. By calibrating predictions via a tempered softmax weighting, we provide a solution to these problems for multiple product-of-expert models, including the generalised product of experts and the robust Bayesian committee machine. Furthermore, we leverage the optimal transport literature and propose a new product-of-expert model that combines predictions of local experts by computing their Wasserstein barycenter, which can be applied to both regression and classification.

==> barycenter-picture.tex <==

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1,scale=0.75]
%uncomment if require: \path (0,248); %set diagram left start at 0, and has height of 248

%Shape: Ellipse [id:dp27925517290252455] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.31 ] (204.5,188) .. controls (204.5,180.27) and (210.77,174) .. (218.5,174) .. controls (226.23,174) and (232.5,180.27) .. (232.5,188) .. controls (232.5,195.73) and (226.23,202) .. (218.5,202) .. controls (210.77,202) and (204.5,195.73) .. (204.5,188) -- cycle ;
%Shape: Ellipse [id:dp4309826736288649] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.31 ] (342.5,191.57) .. controls (342.5,184.71) and (348.54,179.14) .. (355.99,179.14) .. controls (363.45,179.14) and (369.49,184.71) .. (369.49,191.57) .. controls (369.49,198.44) and (363.45,204) .. (355.99,204) .. controls (348.54,204) and (342.5,198.44) .. (342.5,191.57) -- cycle ;
%Shape: Ellipse [id:dp4059390967514078] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.31 ] (199.5,59.5) .. controls (199.5,47.07) and (209.68,37) .. (222.24,37) .. controls (234.81,37) and (244.99,47.07) .. (244.99,59.5) .. controls (244.99,71.93) and (234.81,82) .. (222.24,82) .. controls (209.68,82) and (199.5,71.93) .. (199.5,59.5) -- cycle ;
%Shape: Ellipse [id:dp7535192251881748] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.46 ] (265.77,99.07) .. controls (265.77,94.14) and (270.19,90.14) .. (275.65,90.14) .. controls (281.11,90.14) and (285.53,94.14) .. (285.53,99.07) .. controls (285.53,104) and (281.11,108) .. (275.65,108) .. controls (270.19,108) and (265.77,104) .. (265.77,99.07) -- cycle ;
%Shape: Ellipse [id:dp34375083072282653] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.31 ] (378.63,64.07) .. controls (378.63,56.93) and (384.65,51.14) .. (392.07,51.14) .. controls (399.49,51.14) and (405.5,56.93) .. (405.5,64.07) .. controls (405.5,71.21) and (399.49,77) .. (392.07,77) .. controls (384.65,77) and (378.63,71.21) .. (378.63,64.07) -- cycle ;
%Straight Lines [id:da7514008623234498] 
\draw    (275.65,99.07) -- (360.7,187.57) ;


%Straight Lines [id:da03739705518336711] 
\draw    (275.65,99.07) -- (219.77,186.57) ;


%Straight Lines [id:da9549452522629165] 
\draw    (275.65,99.07) -- (225.81,63.5) ;


%Straight Lines [id:da9004638028003895] 
\draw    (275.65,99.07) -- (387.42,59.57) ;


%Shape: Polygon Curved [id:ds39579201041212486] 
\draw  [fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.11 ] (195.56,33.25) .. controls (210.04,22.67) and (230.82,15.99) .. (254.15,12.29) .. controls (338.67,-1.14) and (456.65,24.43) .. (429.76,45.14) .. controls (395.44,71.56) and (482.09,144.22) .. (516.4,183.85) .. controls (550.72,223.49) and (152.67,247.26) .. (118.35,207.63) .. controls (89.27,174.04) and (116.88,107.24) .. (166.71,57.89) .. controls (175.68,49.01) and (185.36,40.7) .. (195.56,33.25) -- cycle ;

% Text Node
\draw (199.04,93) node  [font=\small]  {$p_1( f\left( \vec x_*\right) |\mathcal{D}^{(1)})$};
% Text Node
\draw (431.83,128.13) node  [font=\LARGE]  {$\mathcal{P}$};
% Text Node
\draw (216.04,213) node  [font=\small]  {$p_2( f\left( \vec x_*\right) |\mathcal{D}^{(2)})$};
% Text Node
\draw (435,195) node  [font=\small]  {$p_3( f\left( \vec x_*\right) |\mathcal{D}^{(3)})$};
% Text Node
\draw (372.04,38) node  [font=\small]  {$p_4( f\left( \vec x_*\right) |\mathcal{D}^{(4)})$};
% Text Node
\draw (328.04,101) node  [font=\small]  {$p_{bar}\left( f\left( \vec x_*\right)\right)$};
% Text Node
\draw (222.04,54) node  [font=\small]  {$\beta _{1}$};
% Text Node
\draw (220,191) node  [font=\small]  {$\beta _{2}$};
% Text Node
\draw (393.07,66.07) node  [font=\small]  {$\beta _{4}$};
% Text Node
\draw (356.99,193.57) node  [font=\small]  {$\beta_{3}$};
\end{tikzpicture}
